The Effects of Correctly Modeling Generator Step-Up Transformer Status in Geomagnetic Disturbance Studies

In order to correctly model the impacts of geomagnetically induced current (GIC) flows, the generator step-up (GSU) transformer status must be properly modeled. In power flow studies, generators are typically removed from service without disconnecting their GSU transformers since the GSU transformer status has little to no impact on the power flow result. In reality, removing a generator from service involves also removing its GSU transformer from service. This difference presents a discrepancy between simulated behavior and system observations during geomagnetic disturbance (GMD) events. This paper presents GMD case studies on 2000-bus and 24,000-bus systems in which reactive power losses and geomagnetically induced currents are compared across scenarios in which the GSU transformers for the disconnected generators are either in-service or out-of-service. The results demonstrate a 3.2 to 15.5 percent error in reactive power losses when the GSU status is modeled incorrectly. Discrepancies of up to 95 A per phase for branch GIC flows and 450 A for transformer neutral GIC flows are also observed and visualized.

==> Sections/ARCHIVED_Analysis_of_Previous_simulations.tex <==
\begin{comment}
\subsection {\color{red}GSU Consideration in Power Flow Analysis\color{black}}
{Case studies could be as follows:
\color{blue}
\begin{itemize}
    \item Analyse GSU OFF/ON Without GMD Scenarios. Take away is to understand there will be changes in the system if we have the wrong model (not considering GSU)
    \subitem  ---Consider Power flow changes, Mvar Losses, Voltage issue..
\color{black}

\end{itemize}
}
\color{black}

\subsection{\color{red}GSU Consideration in GMD Analysis\color{black}}
Two case studies are presented to demonstrate the importance of correct modeling of GSU for an outage of its respected generator during GMD analysis. Each case is broken down into two scenarios. Scenario 1(S1) is one in which a generator is out but its respective GSU is in service. Results will be compared with scenario 2(S2) where both GSU and generator are out of service.

\subsubsection{\color{blue}Case Study 1 (C1)\color{black}}

Here, the contingency is applied such that the generator with the largest MW capacity (569 MW) is out of service. In so doing, the generator connected to bus 189 is disconnected, but its respected GSU transformer (13.8/230 kV) remains operational. The low side of GSU is connected to bus 189 (generator side) while the high side is connected to bus 187 (transmission side).
Figure \ref{fig:C1_Sc1_oneline} shows the one line diagram of the case C1. The neutral GIC can still flow through the high side of GSU (grounded-wye connection) but not through the low side (delta connection). Therefore, in scenario 1, the GIC to bus 187 will come from the high side GSU and the three transmission lines (230 kV) connected to bus 187.

Figure \ref{fig:NeutralGIC_C1_S1} illustrates the neutral GIC on GSU transformer over the course of GMD simulation while GSU is still in service. 
Scenario 2 includes disconnecting the GSU to observe changes in GIC flow and GIC-caused Mvar losses. Table \ref{GICMvarLoss} presents the GIC total MVar loss for the system. Comparing the S1 and S2 for Case 1, it is evident that the GIC total Mvar loss is decreased by 164.6 Mvar when the correct GSU model is considered in S2.

In Figure \ref{fig:C1_BranchGIC}, we show the delta in GIC flow magnitude across the transmission lines connected to the transmission side of GSU for Case 1. This demonstrates the fact that modeling the GSU correctly ( being out of service due to an outage of its respected generator ) affects the GIC flow distribution.

\end{comment}
\begin{comment}

\begin{figure}[t!]
    \centering
    \includegraphics[width = \linewidth]{Figures/C1_Sc1_oneline.png}
    \caption{\color{black} The one-line diagram of case study 1 (\textit{S1}). \color{red}(Increase the size)}
    \color{black}
    \label{fig:C1_Sc1_oneline}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width = \linewidth]{Figures/NeutralGIC_C1_S1.png}
    \caption{\color{black} Neutral GIC flow on GSU transformer (case study 1(\textit{S1}).}
    \color{black}
    \label{fig:NeutralGIC_C1_S1}
\end{figure}

\begin{table}[t]
\captionsetup{justification=centering, labelsep=newline}
\caption{\textsc{GIC Total Mvar Loss}}
\label{tabple}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Description}&\textbf{Scenario \rom{1}}&\textbf{Scenario \rom{2}} \\
 \hline
Case Study 1 &83938&83773\\
\hline
Case Study 2 &83938 &75998\\
\hline
\end{tabular}
\label{GICMvarLoss}
\end{center}
\end{table}





\begin{figure}[t!]
    \centering
    \includegraphics[width= \linewidth]{Figures/C2_Sc1_oneline.PNG}
    \caption{\color{black} The one-line diagram of case study 2 (\textit{S1}). \color{red}(Increase the size)}
    \color{black}
    \label{fig:C2_Sc1_oneline}
\end{figure}

\begin{figure}[!htb]
    \centering
     \setkeys{Gin}{width=\linewidth}
   \subfloat[GIC flow delta on transmission line connected between buses 187 and 188.]{
   \includegraphics{Figures/C1_GIC_Clinton11_Clinton10.png}
        \label{C1_GIC_Clinton11_Clinton10}
        }\hfill
   \subfloat[GIC flow delta on transmission line connected between buses 187 and 121.]{
   \includegraphics{Figures/C1_GIC_Clinton10_Clinton20.png}
    \label{C1_GIC_Clinton10_Clinton20}
   }\hfill
    \subfloat[GIC flow delta on transmission line connected between buses 187 and 45.]{
    \includegraphics{Figures/C1_GIC_Leroy0_Clinton10.png}
        \label{C1_GIC_Leroy0_Clinton10}
    }
    
    %\vspace{16pt}
    \caption{\protect\subref{C1_GIC_Clinton11_Clinton10} and \protect\subref{C1_GIC_Clinton10_Clinton20} and \protect\subref{C1_GIC_Leroy0_Clinton10} depict the difference in magnitude change in the GIC on the lines connected to the transmission side of the GSU for Case Study 1.  }
    \label{fig:C1_BranchGIC}
    
\end{figure} 



\subsubsection{\color{blue}Case Study 2 (C2)\color{black}}
The contingency is defined as a generator failure where the maximum GIC is observed on the GSU transformer the generator was connected to. According to the simulation, the maximum GIC is found on transformer T26, which is connected between buses 93 and 94. It is a 13.8/115 kV GSU transformer. Its respected generator has a capacity of 18 MW. Fig.  \ref{fig:NeutralGIC_C2_S1} represents the neutral GIC appears on GSU 26. 

Table \ref{GICMvarLoss} shows that the GIC total MVAR loss for C1(S2) is higher than for C2(S2). This is caused by the fact that C1's GSU transformer has a higher voltage than C2's, leading to a higher Mvar loss.  
 

\begin{figure}[t!]
    \centering
    \includegraphics[width =\linewidth]{Figures/NeutralGIC_C2_S1.PNG}
    \caption{\color{black} Neutral GIC flow on GSU transformer (case study 2(\textit{S1}) .}
    \label{fig:NeutralGIC_C2_S1}
\end{figure}

\begin{figure}
 \centering
   \setcounter{subfigure}{0}
\subfloat[GIC flow delta on transmission line connected between bus 93 and 191 for Case 2.]
{\includegraphics[width = 0.99\textwidth]{Figures/GIC_Br_C2_Tuscola2_VillaGrove0.png} \label{GIC_Br_C2_Tuscola2_VillaGrove0}
}\\
\subfloat[GIC flow delta on transmission line connected between bus 93 and 27 for Case 2.]
{\includegraphics[width = 0.97\textwidth]{Figures/GIC_Br_C2_Tuscola2_Windsor0.png} \label{GIC_Br_C2_Tuscola2_Windsor0}
}\\

\subfloat[GIC flow delta on transmission line connected between bus 93 and 11 for Case 2.]
{\includegraphics[width = 0.97\textwidth]{Figures/GIC_Br_C2_Tuscola2_Lovington0.png} \label{GIC_Br_C2_Tuscola2_Lovington0}

}
    \vspace{-2mm}
     \caption{\protect\subref{GIC_Br_C2_Tuscola2_VillaGrove0} and \protect\subref{GIC_Br_C2_Tuscola2_Windsor0} and \protect\subref{GIC_Br_C2_Tuscola2_Lovington0} depict the difference in magnitude change in the GIC on the lines connected to the transmission side of the GSU 26 for Case Study 2.  }
    \label{C2_BranchGIC}
\end{figure}
\end{comment}
\color{black}
\color{blue}
